Interior-proximal primal-dual methods

We study preconditioned proximal point methods for a class of saddle point problems, where the preconditioner decouples the overall proximal point method into an alternating primal--dual method. This is akin to the Chambolle--Pock method or the ADMM. In our work, we replace the squared distance in the dual step by a barrier function on a symmetric cone, while using a standard (Euclidean) proximal step for the primal variable. We show that under non-degeneracy and simple linear constraints, such a hybrid primal--dual algorithm can achieve linear convergence on originally strongly convex problems involving the second-order cone in their saddle point form. On general symmetric cones, we are only able to show an $O(1/N)$ rate. These results are based on estimates of strong convexity of the barrier function, extended with a penalty to the boundary of the symmetric cone.

==> texbase/highlightname.tex <==
%\addbibresource{\jobname.bib}
\newcommand*{\mknamesignature}[5]{\edef#1{(#2|#3|#4|#5)}}
\mknamesignature{\highlightname}{DISABLEDValkonen}{DISABLEDTuomo}{}{}
\def\highlightfamily{Valkonen}
\def\ancientversion{2.8a}
% mbox needed to not make next character automatically  upper case
\providecommand{\shortform}{\mbox{T.\,V.}}
\makeatletter

\ifdefequal{\abx@version}{\ancientversion}{
	\DeclareNameFormat{labelname}{%
	  \begingroup
	  \mknamesignature{\currentsignature}{#1}{#3}{#5}{#7}%
	  \ifdefequal{\highlightname}{\currentsignature}%
	    {\let\mkbibnamefirst=\@gobble%
	     \def\mkbibnamelast{\shortform\@gobble}%
	     \let\mkbibnameprefix=\@gobble%
	     \let\mkbibnameaffix=\@gobble}%
	    {\let\mkbibnamefirst=\@gobble}%
	  \ifcase\value{uniquename}%
	    \usebibmacro{name:last}{#1}{#3}{#5}{#7}%
	  \or
	    \ifuseprefix
	      {\usebibmacro{name:first-last}{#1}{#4}{#5}{#8}}
	      {\usebibmacro{name:first-last}{#1}{#4}{#6}{#8}}%
	  \or
	    \usebibmacro{name:first-last}{#1}{#3}{#5}{#7}%
	  \fi
	  \endgroup
	  \usebibmacro{name:andothers}%
	}
}{
	\DeclareNameFormat{labelname}{%
	  \nameparts{#1}%
	  \begingroup%
	  \mknamesignature{\currentnamex}{\namepartfamily}{\namepartgiven}{\namepartprefix}{\namepartsuffix}%
	  \ifdefstrequal{\highlightname}{\currentnamex}%
	    {%
	      \usebibmacro{name:delim}{\shortform}%
	      \shortform%
	    }{%
	      \usebibmacro{name:family}
	           {\namepartfamily}
	           {\namepartgiven}
	           {\namepartprefix}
	           {\namepartsuffix}%
	    }%
	  \endgroup%
	  \usebibmacro{name:andothers}
	}
}
\makeatother

\DeclareNameAlias{default}{labelname}


==> texbase/symbols-mna.tex <==

\newcommand{\mna}{\phi}
\newcommand{\plusmna}{\oplus}
\newcommand{\minusmna}{\ominus}
\newcommand{\iprodmna}{\odot}
%\DeclareMathOperator{\plusmna}{\hat +}
%\DeclareMathOperator{\minusmna}{\hat{--}}
%\DeclareMathOperator{\iprodmna}{\hat \times}
\newcommand{\Rmna}{\R_\mna}
\newcommand{\maybeeq}{\stackrel{?}{=}}
\newcommand\rhodom\sqsubset
\newcommand\rhodominv\sqsupset
\newcommand\rhodomneq{\sqsubset_{!}}
\newcommand\rholub\sqcup
\newcommand\rhoglb\sqcap
\newcommand{\sumop}{\biguplus}
\newcommand{\sumz}{\biguplus}
\newcommand{\plusz}{\uplus}
\newcommand{\minusz}{\uminus}
\newcommand{\pz}{\zeta}

